OpenFunction: Data Plane Abstraction for Software-Defined Middleboxes

The state-of-the-art OpenFlow technology only partially realized SDN vision of abstraction and centralization for packet forwarding in switches. OpenFlow/P4 falls short in implementing middlebox functionalities due to the fundamental limitation in its match-action abstraction. In this paper, we advocate the vision of Software-Defined Middleboxes (SDM) to realize abstraction and centralization for middleboxes. We further propose OpenFunction, an SDM reference architecture and a network function abstraction layer. Our SDM architecture and OpenFunction abstraction are complementary to existing SDN and Network Function Virtualization (NFV) technologies. SDM complements SDN as SDM realizes abstraction and centralization for middleboxes, whereas SDN realizes those for switches. OpenFunction complements OpenFlow as OpenFunction addresses network functions whereas OpenFlow addresses packet forwarding. SDM also complements NFV in that SDM gives NFV the ability to use heterogenous hardware platforms with various hardware acceleration technologies.

==> chen/abstract.tex <==
\begin{abstract}
The state-of-the-art SDN abstractions only focus on packet forwarding in switches, and these abstractions lack the ability to implement middlebox data plane functionalities.
%
In this paper, we propose a data plane abstraction called \sys~to realize the vision of SDN for middleboxes, complementing what OpenFlow/P4 achieve for switches.
%
By exposing an extensible actions abstraction to the control plane, \sys~decouples the middlebox program from the underlying data plane devices (\emph{target independence}) and also supports building any new packet actions in a target-independent way (\emph{full extensibility}) for the southbound interface of Network Function Virtualization.
%
Build upon \sys, we develop a control centralization model:
%
a logically centralized NFV controller performs resource allocation according to a flow's middlebox service chain, and coordinates with the forwarding plane authority (\ie, an OpenFlow controller) to enforce it.
%
We fully implemented a working \sys~system including one NFV controller, three \sys~enabled boxes, and a number of non-stateful/stateful NFV middleboxes.
%
The evaluation results show that we successfully achieve our design goal: data Plane abstraction and control plane centralization for Network Function Virtualization.
%
%By these proof-of-concept systems, we verify the proposed abstraction, and get the first-hand estimate of achievable performance.

\end{abstract}


==> chen/actions.tex <==
\presec \section{Abstraction Design} \label{sec:actions} \postsec

%\vspace{-0.1in}
\presub \subsection{Abstraction Specification} \postsub
\label{sec:actions:specification}
%
\sys~uses a Click-style script for specification: an example of IPSEC middlebox data plane is shown in Algorithm~\ref{code:ipsec}.
%
Analogous to Click, the action parameters are enclosed by bracket.
%
Hereby is the brief example description: from incoming link, only IP packets are accepted and the ethernet headers are removed; 
%
each packet is then encapsulated with an ESP  header, and encrypted with the EBC algorithm; 
%
the new outer IP tunnel header is added and IP checksum is updated;
%
after the MAC header are added, the packet is forwarded to the outgoing link. 

\begin{algorithm} [t]
\caption{\textbf{IPSEC Specification (one way)}}\label{code:ipsec}
FromDevice(1)->ExactMatch(PROTO\_IP,-)
->DecapHeader(14)->ESPEncap->Aes(EBC)
->IPsecEncap->ChangeSrcIP(IP\_SRC)
->ChangeDstIP(IP\_DST)->SetIPChecksum
->EncapHeader(MAC\_DEST, MAC\_SRC, PROTO\_IP)
->ToDevice(2)
\end{algorithm}

%
To carefully tradeoff composability and optimizability, we analyze and implement a number of middleboxes such as NAT, IPSec, and IDS, and design a suite of actions that we classify into the following four categories:
%
\begin{itemize}
\item \emph{Packet Receive/Send:} These actions receive/send packets from/to either hardware/virtualized NICs, or specific memory locations (\eg, FromDevice and ToDevice in the IPSEC example ).

\item \emph{Flow Classification:} This category consists of actions based on the following four matches: exact-match (\eg, used in the IPSEC example), longest-prefix-match (\eg, used in FIB), first-match (\eg, used in ACL), and pattern-match (\eg, used in DPI).

\item \emph{Flow Scheduling:} A flow scheduling action takes multiple flows as input, and outputs one combined stream of traffic. Example flow scheduling operations include strict priority (SP) and weighted round robin (WRR).

\item \emph{Straight Operations:} These actions perform a single packet processing such as changing the length of a packet, either at the head (\ie, Encap/Decap) or the tail (\ie, Pad/Unpad), and modifying a field or the metadata of a packet (\ie, decreasing the IP TTL value and setting the ECN bit are two actions).
\end{itemize}
%
The attributes of an action can be set either at the configuration phase, or at run-time.
%
Stick to the IPSEC example, for a given IPSEC tunnel, the IP\_SEC/IP\_DST attributes of ChangeSrcIP/ChangeDstIP actions are set at the configuration phase as parameters
%
While for the ESPEncap action, its security index SPI and replay parameter RPL should be negotiated by the control plain at run-time;
%
the IPSEC DP process leaves the two attributes unset at first, and lets the CP process performs negotiation before setting the attribute value.

%%
As the target of action operations, a packet class consists of three types of data: fields, metadata, and properties.
%
The metadata is a piece of memory associated with a packet and is used to store modifiable information about the packet, such as the ID of the physical port from which the packet is received.
%
The properties means some non-modifiable information about the packet, such as the packet size.
%
Although some properties of a packet may change after certain actions, \eg, the length of a packet changes after Encap/Decap, the properties of a packet cannot be written or modified by action functions directly.
%
Table \ref{table:middleboxes} summaries the accessibility of packet data.

\begin{table}[htb]
\begin{center}
\vspace{-0.05in}
\scalebox{1}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline Targets & \multicolumn{3}{|c|}{Packet} & \multicolumn{2}{|c|}{Action} \\
\hline & Field & Metadata &  Property &  Attributes & Event \\
\hline
Read  & Yes &  Yes  &  Yes &  Yes  &  No \\
\hline
Write & Yes &  Yes  &  No  &  Yes  &  Yes \\
\hline
\end{tabular}}
\vspace{-0.1in}
\caption{Summary of data access}\label{table:middleboxes}
\vspace{-0.15in}
\end{center}
\end{table}

%
To prevent the exact fate of OpenFlow's vertical integration, we do not enforce any standard action.
%
Instead, a set of actions are \emph{recommended}; and for each such action, a default implementation written in \sys~pseudo language (next part) is provided together,
%
An \sys~box can flexibly choose the action to optimize by exploiting their underlying hardware acceleration capabilities.
%
For the actions whose optimized implementation is not available at the box, the default pseudo code can be used, like user-defined action.

Furthermore, we allow \sys~boxes to provide multiple implementations of the same action: for example, one version is CPU based and another version is GPU based. 
%
The controller can dynamically determine which version to load/unload based on the availability of network resources and the processing requirements of
flows at run time. 
%
Later in Section~\ref{sec:scheduling}, we consider this flexibility in formulating and solving the service chain scheduling problem.

\presub \subsection{Pseudo Language} \postsub
\label{sec:actions:language}
%
We propose a platform-independent pseudo language that allows SDM developers to design arbitrary middlebox data plane functionality, and supported by any \sys~enabled device.
%
The vendor of an \sys~box needs to provide a source-to-source translator, which takes a pseudo C program as its input and outputs a native program that exploits the hardware acceleration strength of the box.
%
The output platform-dependent program is further compiled into executable components using the box's native compiler.
%
As a proof-of-concept, shown in Section~\ref{sec:system}, in our prototype system an action class can be translated either to a platform-dependent C/C++ program such as a Click element, or a FPGA block (in Verilog).

%%
We now introduce the packet field abstraction that the pseudo programs operate on.
%
The whole packet is assumed to be stored in a continuous memory location as shown in Figure \ref{fig:data}.
%
There is infinite headroom/tailroom before/after the packet data.
%
Such spaces are reserved for actions that change packet length (\ie, Encap/Decap and Pad/Unpad).
%
We also assume the existence of a mandatory preprocessing step, which marks the start offset of link/network/tranport/app layers (if they exist).
%
Each field is a continuous range of bytes in a packet memory range, defined by a tuple \texttt{(header, offset, type)} and can be attached with a name.
%
For example, IP checksum can be defined as a field starts at the 10th bytes offset of the network header by the \texttt{FIELD} keyword.
%
The length is automatically determined by its data type \texttt{UNIT16}.
%
Note that a special type is \texttt{DATA}, which represents a raw array of bytes.

\begin{figure}[htbp]
\vspace{-0.1in}
\centerline{\includegraphics[width=1\linewidth]{figure/data}}
\vspace{-0.1in}
\caption{Abstraction of packet field} \label{fig:data}
\vspace{-0.1in}
\end{figure}

%%
The metadata of a packet is accessed as a named object (with keyword \texttt{META}).
%
In OpenFunction, a \texttt{(type, length)} tuple defines a specific metadata object.
%
The \texttt{length} configuration is required only when the \texttt{type} is \texttt{DATA}.
%
This design provides the system with the freedom to arrange a meta object in its metadata memory.
%
Packet properties (with keyword \texttt{PROP}) and action attributes (with keyword \texttt{ATTR}) are also accessed as named objects.
%
Note that packet properties are limited to a small set of intrinsic packet characteristics and read-only to program.
%
The additional feature of an attribute is that it can be read/written by another action or the control plane.
%
Each event object is a continuous raw array of bytes.
%
It is up to the action developer to decide the content of the event.

A key design decision is to separate packet access (Table \ref{table:middleboxes}) codes and normal codes.
%
More specifically, we use character "@" at the start of a line to denote a data access line.
%
Following the "@" letter, there should either be a packet variable definition of \texttt{FIELD}, \texttt{META},  \texttt{PROP} or \texttt{ATTR}, or \texttt{LOAD}/\texttt{STORE} to access the data.
%
Currently, we do not support direct algorithmic operations over packet data variables; they are used to denote the physical locations in the packet.
%
Instead, we first load them into local variables, perform calculation, and then store them back.
%
The benefit is that all non-data-access codes can be written as normal C codes.

%
Algorithm \ref{alg:SetIPChecksum} shows an example pseudo program.
%
This user-defined \emph{SetIPChecksum} action accepts an incoming IP packet and calculates and sets its IP checksum field; here the action assumes that the incoming packets are with MAC headers.
%
As an example, the \emph{iphlen} is defined first (Line 1), and loaded into a local variable \emph{hlen} before used (Line 5).
%

\begin{algorithm}
\caption{\textbf{SetIPChecksum (User Defined)}}\label{alg:SetIPChecksum}
\KwIn{Packet \texttt{P}}
\KwOut{\texttt{P} with IP Checksum field set}
\BlankLine
@ FIELD \texttt{iphlen}   NETWORK 0  UINT8 \;
@ FIELD \texttt{ipcsum}   NETWORK 10 UINT8 \;
@ FIELD \texttt{ipheader} NETWORK 0  DATA \;
\BlankLine
unsigned char \texttt{hlen}\;
@ LOAD \texttt{iphlen} \texttt{hlen} \;
\texttt{hlen} = \texttt{hlen} \& 0x0f\;
\texttt{hlen} = \texttt{hlen} << 2\;
\BlankLine
@ STORE \texttt{ipcsum} 0 \;
\BlankLine
unsigned int \texttt{sum}=0\;
unsigned short \texttt{hoffset}=0\;
unsigned short \texttt{tempshort}=0\;
\While {\texttt{hoffset} < \texttt{hlen}}{
    \{
    \ @ LOAD \texttt{ipheader} \texttt{tempshort} \texttt{hoffset} UINT16 \;
    \texttt{hoffset} = \texttt{hoffset} + 2\;
    \texttt{sum} = \texttt{sum} + \texttt{tempshort}\;
    \}
}
\BlankLine
unsigned int \texttt{tempint} = 0\;
\texttt{tempint} = \texttt{sum} \& 0xffff0000\;
\While {\texttt{tempint} != 0}{
\{
\texttt{sum} = \texttt{sum} \& 0xffff\;
\texttt{tempint} = \texttt{tempint} $\gg$ 16\;
\texttt{sum} = \texttt{sum} + \texttt{tempint}\;
\texttt{tempint} = \texttt{sum} \& 0xffff0000\;
\}
}
\BlankLine
sum = $\sim$sum\;
@ STORE \texttt{ipcsum} \texttt{sum} \;
\end{algorithm}



==> chen/conclusion.tex <==
\presec \section{Conclusions} \label{sec:conclusions} \postsec
%% Point: OpenFunction realized centralization
Our OpenFunction architecture realized the centralization vision for middleboxes by the logically centralized OpenFunction controller.
%
As it is well understood that centralization in OpenFlow brings a long list of benefits to packet forwarding such as flexible path selection, better load balancing, finer-grained network control, less configuration errors, higher manageability, and increased reliability and security,  centralization in OpenFunction brings many benefits to middlebox functionalities.
%
For example, the global view that a CP process obtains from the events generated by the group of DP processes that it manages helps the CP to make better informed decisions.
%
For example, an IDS CP process can perform correlation analysis on the events from its DP processes to better identify attack activities.
%
For another example, the ability that a CP process can issue commands to its DP processes allows the CP to orchestrate the DP processes to collaboratively accomplish some tasks.

%% Point: OpenFunction realized abstraction
Our OpenFunction architecture realized the abstraction vision for middleboxes by the OpenFunction abstraction layer.
%
Through abstraction, for middleboxes, we decouple their hardware and software as well as their control plane and data plane.
%
This abstraction layer eliminates hardware vendor lock-in because the underlying hardware architecture and vendor are transparent to DP processes.
%
It also eliminates software vendor lock-in because any DP software can run on any OpenFunction boxes.
%
This abstraction layer supports hardware/software heterogeneity and promotes hardware/software innovation as the abstraction layer can be implemented in a variety of hardware/software technologies such as ASIC, multi-core, FPGA, and GPU.
%
This lowers the middlebox market barrier because as long as a hardware device supports the abstraction layer, it can immediately support DP processes and thus can be immediately deployed on existing networks to work with existing devices.
%
This abstraction layer also significantly improves the programmability of middlebox functionalities because a DP developer does not need to implement those common operations in packet processing.
%
From the software engineering perspective, this abstraction layer promotes software reuse.
%
This will significantly shorten the time-to-market cycle.

%% Point: OpenFlow + OpenFunction support management
%% Camera ready version: comment off this paragraph
OpenFunction, together with OpenFlow, helps to support the vision of service oriented network management.
%
While OpenFlow makes switches easier to manage, currently middleboxes are still notoriously difficult to manage because the hardware and software of those middleboxes are often tightly coupled and different middleboxes of different vendors often have different management interfaces.
%
Service oriented network management means to automate the translation from high-level service oriented network management requirement to low-level network device configurations.
%
For example, a high-level service oriented network management requirement can be to ``allocate 10G bandwidth between two networks and to ensure that all traffic between the two networks to pass through an IDS''.
%
While translating this high-level requirement to network device configurations in today networks is a complex, laborious, and error prone process, it can be easily done in OpenFunction+OpenFlow by the following two automated steps.
%
First, we use OpenFlow to find an appropriate path between the two networks where each switch on the path has at least 10G bandwidth and the path contains at least one OpenFunction enabled device.
%
Second, on that OpenFunction enabled device, the OpenFunction controller
%disables the SDM DP process running and
starts a new IDS DP process.


==> chen/evaluation.tex <==
\presec \section{Evaluation} \label{sec:evaluation} \postsec
\presub \subsection{Abstraction} \postsub
At the first test, we provide the \sys~specification of the data plane of each SDM.
%
For each SDM, the same \sys~specification is used.
%Here we evaluate the throughput performance of the SDM applications implemented by our abstraction.
%
We test with both small size packets (60 bytes) and large size packets (1400 bytes).
%
Table~\ref{table:throughput} shows the throughput performance.
%

%
First we focus on non-stateful SDMs: NAT and IPSEC.
%
In almost all setting, DPDK box gets higher throughput than Netmap-based box.
%
This demonstrates that, even with the same OpenFunction abstraction implementation and the same hardware, the performance
actually relies on underlying systems.
%
In turn, the FPGA box is always better than DPDK.

\noindent\textbf{Key Takeaway 1~~} Our \sys~abstraction accommodates vendor differentiation with the same code across heterogeneous systems, which is beneficial for the NFV community.

\begin{table}[htb]
\caption{Throughput of \sys~middleboxes}\label{table:throughput}
\begin{center}
\scalebox{1}{
\begin{tabular}{|c|c|c|c|c|}
%\hline & \multicolumn{3}{|c|}{NAT} \\
\hline & Netmap & DPDK & FPGA &  FPGA-C \\
\hline
\hline
NAT Small  & 1.78 Gbps & 1.84 & 1.64 Gbps &  0.24 Gbps\\
\hline
NAT Large &  7.84 Gbps & 9.96 & 9.34 Gbps  &  0.72 Gbps \\
\hline
IPSEC Small  & 0.59 Gbps & 1.2 & 2.61 Gbps &  X Gbps\\
\hline
IPSEC Large &  0.93 Gbps & 2.8 & 9.35 Gbps  &  X Gbps \\
\hline
\hline
FW Small  & X Gbps & N/A & N/A &  N/A\\
\hline
FW Large &  X Gbps & N/A & N/A  &  N/A \\
\hline
IPS Small  & X Gbps & N/A & N/A &  N/A\\
\hline
IPS Large &  X Gbps & N/A & N/A  &  N/A \\
\hline
\end{tabular}}
\end{center}
\end{table}

Next, we replace the \emph{SetIPChecksum} and \emph{SetTCPChecksum} actions in the specification with user defined versions (written in \sys~language and translated).
%
The performance overhead caused by user defined versions is negligible: for these software-based boxes, without special acceleration treatment, the C compiler performs most of the optimization work; for such an action, the efficiency of a translated version could be similar to the implemented version.
%
%The results of firewall and IPS are similar.

As a comparison, shown in Table~\ref{table:throughput}, in FPGA platform, the performance gap between optimized implementation and \sys~language generated version (\ie, FPGA-C)is huge (10x in this case).
%
The reason is that FPGA enables a large space of optimization performed by the programmer.
%
As a concrete example, for NAT function, the programmer may choose to calculate the checksum at line rate, without the need to receive the whole packet.

\noindent\textbf{Key Takeaway 2~~} The performance of SDM data plane actions, if generated from \sys~pseudo language, are dominated by the nature of the system.

We also present the results for two stateful SDMs: FW and IPS.
%
Their performance is comparable to non-stateful SDMs.

\noindent\textbf{Key Takeaway 3~~} \sys~abstraction has the potential to support various stateful firewalls.


\presub \subsection{Centralization} \postsub
%


\noindent\textbf{Key Takeaway 4~~} \sys~abstraction has the potential to support various stateful firewalls.

%
We consider two scenarios to evaluate OpenFunction data plane overhead:
(1) time it takes to start/stop a data plane process in the service chain; and
(2) additional path delays due to our chain enforcement inside a box.
%
In the first case, we are interested in understanding how much delay is incurred when a new service chain or SDM DP is added or removed from the network.
%
To evaluate, we use a small topology in Figure~\ref{fig:topo} with DPDK middleboxes and generate TCP flows between source and destination.
%
We initiate flows on path 1 and path 2 which initiates flow rule installation in the switches along the datapath and calculate datapath setup times.
%
Our evaluation shows that it takes less than 100\,msec to add a new datapath or service chain in the network.
%
%Note that adding a service chain in the MB is similar to adding new datapath in the network.
%
In the second case, we are interested in understanding the additional delays caused by enforcing service chains in the MB's.
%
Our evaluations shows that it adds less than 20 usec per SDM DP in the service chain.

\begin{figure}[htbp]
\vspace{-0.1in}
\centerline{\includegraphics[width=01\linewidth]{figure/topology}}
\caption{Test Topology}\label{fig:topo}
\vspace{-0.1in}
\end{figure}

%
In this case, we are interested in knowing the responsiveness of the controller to adapt to dynamic network conditions and
we measure the time required to reconfigure the network in case of SDM DP failure or traffic overload in some of the service chains.
%
We consider topology shown in Figure~\ref{fig:topo} with DPDK middleboxes and use Iperf \cite{iperf} to generate TCP flows between source and destination.
%
We first initiate flows on $path 1$ and $path 2$ by install rules in the switches along the datapath and distribute load evenly across the two paths.
%
Next, we bring down the switch in $path 2$ and observe how quickly network converges to the stable state and diverts traffic to $path 1$.
%
Our evaluation shows that network takes less than 200\,msec to converge to a stable state and reconfigure flows to use other paths.
%
We also dynamically change the datapaths, to replicate the SDM insertion and deletion scenarios, in our topology to steer network traffic through different paths and our evaluation shows that the network quickly adapts to these changes without any drop in the flow throughput.

\noindent\textbf{Key Takeaway 5~~} \sys~abstraction is flexible and has light overhead.


==> chen/introduction.tex <==
%\vspace{-0.1in}
\presec \section{Introduction} \label{sec:introduction} \postsec
%
The vision of Software-Defined Networking (SDN) is two-fold: \emph{abstraction} and \emph{centralization}.
%
Abstraction means to use common interfaces for heterogenous network devices of different vendors/architectures and to implement the functionalities demanded by the control plane.
%
Centralization means to use a logically centralized controller in the control plane to obtain a global view of a network and to manage network resources and functionalities in an orchestrated and flexible manner.
%
Abstraction and centralization help SDN to achieve its two goals: \emph{breaking device vendor lock-in} and \emph{supporting network innovation}.
%
Abstraction allows third-party software to run on all SDN compliant network devices.
%
In contrast, traditional network devices are black boxes where both hardware and software are tightly coupled as they are typically from the same vendor, which leads to both network ossification and vendor lock-in.
%
Centralization allows network resources and functionalities to be dynamically and flexibly managed.

%% Point: OpenFlow is not enough.
The state-of-the-art SDN abstractions, \ie, OpenFlow and P4~\cite{OpenFlow08Nick, OpenFlowSpecification15, bosshart2014p4}, only partially realized this vision of SDN as they focus on packet forwarding in switches.
%
However, a data communication network mainly consists two types of devices, \emph{switches} and \emph{middleboxes}.
%
Switches (including routers in the broader sense) provide packet forwarding.
%
Middleboxes provide a wide variety of networking and security functionalities such as Network Address Translation (NAT), Load Balancers (LB), firewalls (FW), WAN optimizers, proxies, IPSec gateways (VPN), and network Intrusion Detection/Prevention Systems (IDS/IPS).

OpenFlow/P4 match-action abstractions are fundamentally limited in implementing middlebox data plane functionalities.
%
Firstly, they have only minimum number of actions that can apply to packets.
%
Some middleboxes, such as IPSec VPN, need to perform complex payload actions such as encryption and decryption.
%
To address the limitations in the action abstraction, OpenFlow standards have kept adding new actions.
%
Obviously, this is not a sustainable solution as packet processing actions can never be exhaustively standardized (\eg, invention of a new encryption algorithm).
%
Furthermore, frequent standardization of new action abstraction in OpenFlow/P4 would lead to frequent redevelopment of software/hardware, which results in vertically integrated hardware-software that must be replaced all together while upgrading network~\cite{Anwer2013}.
%
Secondly, their match abstractions have limited expression power due to the fixed number of fields that they extract only from packet headers.
%
Some middleboxes, such as application firewalls and IPSes, need to extract arbitrary application protocol fields or even signatures from packet payload~\cite{AlexFlowSifterJSAC14}.
%
Lastly, the table abstraction is fundamentally incapable of modeling the function of scheduling.
%
Scheduling is essential to implement Quality-of-Service (QoS), which is further essential for many middlebox functionalities.
%
This inability is because the table abstraction performs splitting an aggregate flow into multiple flows whereas scheduling performs merging multiple flows into an aggregate flow.
%
In some sense, a table and a scheduler perform totally opposite functionalities, and one cannot model the other.

%
In this paper, we propose a data plane abstraction called \emph{OpenFunction} to realize the vision of SDN for middleboxes, complementing what OpenFlow/P4 achieve for switches.
%
More specifically, \sys~targets the southbound interface for Network Function Virtualization (NFV) architectural framework (detail in Section~\ref{sec:related}).
%
In designing \sys, we have two main goals:
%
\begin{itemize}
\item \emph{target independence.~~} A middlebox application programmer should not know the details of the underlying data plane devices, be it a multi-core CPU, a network processor, a FPGA, a GPU or an ASIC chip.
\item \emph{full extensibility.~~} Besides provided actions, a middlebox programmer should be able to build any new packet actions also in a target-independent way.
\end{itemize}
%

To meet these requirements, \sys~exposes an extensible abstraction of \emph{actions} to the control plane:
%
despite the underlying heterogeneous hardware platform and features, a common (and gradually extensible) library of recommended middlebox actions should be provisioned by every \sys~enabled hardware platform; user-defined or not-yet-implemented (by the platform) actions should be composed by writing in a platform-independent pseudo language, which in turn can be compiled to target-dependent modules and executed by a specific device.
%
From the control plane's point of view, each middlebox's data plane is defined by a specification, which defines \emph{how packets are operated by a directed acyclic graph of actions} in the data plane.
%
Similar to P4 in forwarding, the \sys~specification raises the level of abstraction in functionality: the programmer gives a target-independent data plane specification; the device translates the specification into its target-dependent processing program.
%
Build upon \sys, we develop a control centralization model:
%
a logically centralized NFV controller performs resource allocation according to a flow's middlebox service chain, and coordinates with the forwarding plane authority (\ie, an OpenFlow controller) to enforce it.

%% Technical Challenges and Solutions
There are three main challenges.
%
The first key technical challenge is on designing the abstraction layer for the data plane:
%
we need to carefully tradeoff between fine and coarse abstraction granularity.
%
Finer abstraction granularity leads to better programmability but worse performance due to reduced optimization opportunities.
%
Coarser abstraction granularity leads to better performance but worse programmability due to reduced programming flexibilities.
%
To address this challenge, we analyze and implement a number of middleboxes and decompose them to a set of atomic action where each action is self-contained and functionally independent.
%
We categorize these atomic actions to four categories: packet receive/send, flow classification, flow scheduling, and straight operations.
%

Second, we need to achieve full programming extensibility, \ie, we want our suite of atomic actions to be extensible to build any new network functionality.
%
To address this challenge, we design a pseudo programming language targeting source-to-source translation.
%
An \sys~enabled device needs to provide a compiler, which first performs a source-to-source translation from a platform-independent pseudo program to a platform dependent
program, which is further compiled into native code using a platform dependent third-party compiler/library.

%%
Yet another technical challenge is service chain scheduling where given a service chain that a flow needs to traverse, the controller chooses a sequence of middlebox data plane processes (running on one or more \sys~boxes) to form the service chain.
%
The scheduling not only needs to satisfy the three requirements of service chain constraints, device resource constraints, and flow conservation, but also needs to do it in a load balancing way to minimize the maximum utilization of the resources in candidate devices.
%
To address this challenge, we formulate service chain scheduling as a NP-Hard problem, and proposed both offline and online scheduling algorithms.

%%Implementation and evaluation
We fully implemented a working \sys~system including one NFV controller, three \sys~enabled boxes, and a number of non-stateful/stateful NFV middleboxes.
%
The evaluation results show that we successfully achieve our design goal: data Plane abstraction and control plane centralization for Network Function Virtualization.

The rest of paper proceeds as follows.
%
We first review background and motivation in Section~\ref{sec:related}.
%
The overview of our design is presented in Section~\ref{sec:overview}.
%
Then, we introduce our middlebox data plane abstraction in Section~\ref{sec:actions}, and control plane service chain scheduling
algorithms in Section~\ref{sec:scheduling}.
%
The implementation of the prototype system is described in Section~\ref{sec:system}.
%
Extensive evaluation results are demonstrated in Section~\ref{sec:evaluation}.
%
We conclude our paper in Section \ref{sec:conclusions}.



==> chen/overview.tex <==
\presec \section{Overview} \label{sec:overview} \postsec
%\presub \subsection{System Model} \postsub
%% Point: OpenFunction realized abstraction
\begin{figure*}[htbp]
\centerline{\includegraphics[width=1\linewidth]{figure/architecture}}
%\vspace{-0.15in}
\caption{Architecture Overview} \label{fig:architecture}
%\vspace{-0.15in}
\end{figure*}
%
In \sys~model of NFV application scenarios, there is a number of \sys~enabled \emph{boxes} distributed across the network, and a logically centralized \emph{controller} realizes control centralization for NFV.
%
For NFV middleboxes, their data planes are running on \sys~enabled boxes, and their control planes are running on a number of general purpose x86 machines.
%
To overview the design, hereby we present the views from three different perspectives: data plane, middlebox and the whole system.


%%
\noindent\textbf{Data Plane View:}
%
To achieve both \emph{target independence} and \emph{full extensibility}, \sys~exposes an extensible abstraction of \emph{actions} to the control plane as shown in Figure~\ref{fig:architecture}~(a).
%
The semantics of an action is to take a packet as its input, execute its action, and either push the packet to the downstream action or
wait for the downstream action to pull the packet.
%
\sys~abstraction is action oriented, similar to the object oriented programming paradigm.
%
Each action object is an instance of an action class.
%
An action class represents a self-contained and functionally independent packet processing unit, such as decreasing the TTL field, calculating the TCP checksum, \etc.
%
An action class consists of data members, which we call \emph{attributes}, that can be changed.
%
For example, a \texttt{PacketCounter} action may need to update its counter attribute whenever a packet passes through this action.
%
The actions may also need to send an event to the corresponding control plane.
%
For example, a \texttt{TCPSyncNotifier} action may need to send a TCP sync event whenever a TCP sync packet passes through this action.

There are two kinds of actions: \emph{provisioned} and \emph{composed}.
%
Despite the underlying heterogeneous hardware, a common (and gradually extensible) library of recommended middlebox actions are provisioned by every OpenFunction enabled hardware platform, thus target independence is achieved.
%
User-defined or not-yet-implemented (by the platform) actions can be \emph{composed} by writing in a platform-independent pseudo language, which in turn can be compiled to target-dependent
modules and executed by a specific device.
%
As a result, full extensibility is supported.

%%
\noindent\textbf{Middlebox View:}
%
As illustrated in Figure~\ref{fig:architecture}~(b), each network function (\eg, NAT, LB, or FW) is accomplished by a Control Plane (CP) process running on a x86 machine and a (group of) Data Plane (DP) processes running on \sys~boxes.
%
For each network function, its data plane specification is an \emph{action graph}, which is a directed acyclic graph (DAG) and each node in the DAG is an action.
%
A DP process has a local view of the network, and its main role is to process data plane packets.
%
Based on the processed traffic, it may sends events to its CP process, and receives commands from its CP process.
%
The CP process has a global view (via the controller) and its main role is to make well-informed decisions for the group of DP processes that it manages, according to its middlebox functionality.
%
It receives events from DP processes, performs analyses, makes decisions, and sends commands to DP processes to enforce its decisions.
%
We call a CP process together with its group of DP processes a \emph{Software-Defined Middlebox} (SDM).

Using \sys~, from the perspective of an SDM developer, the burden of defining the data plane is significantly reduced: mostly the only requirement is to compose the flow processing graph via a simple \sys~specification (Sec.~\ref{sec:actions:specification}).
%
The main focus of the developer is the control plane CP process.
%
In the rare case that a required packet action may not be supported, the developer could implement the processing logic via \sys~language~(Sec.~\ref{sec:actions:language})

%%
\noindent\textbf{System Diagram:}
Figure~\ref{fig:architecture}~(c) contains the major components of a \sys~enabled system.
%
The main job of the NFV controller is to perform management, scheduling and service chain enforcement.
%
A SDM CP process provides, to the controller, its flows with a required middlebox service chain.
%
The controller monitors resource (such as CPU, memory, or a specific acceleration card) utilization and executes an service chain scheduling algorithm; it then coordinates with the forwarding plane authority (\ie, an OpenFlow controller) to enforce the chain.
%
Each \sys~enabled device has a middleware layer called a \sys~shim layer, which manages all DP processes running on the device, such as installs a DP, starts a DP
process, and terminates a DP process. 
%
The shim layer is fully controlled by the controller and the controller monitors the resource unitization through it.

%%
Note that service chains needs to be enforced both across and inside boxes.
%
A Openflow controller still controls the forwarding between devices centrally: the controller sends flow steering instructions to the Openflow controller.
%
A dedicated IO process of the shim layer steers flows among functions according to their service chain.
%%
%An example is shown in Figure~\ref{fig:chain}: a flow needs to traverse a service chain $SDM~1\rightarrow SDM~2 \rightarrow SDM~3$; $SDM~1$ is computationally intensive; it has a GPU version in Node~1, and a CPU version in Node~2.
%%
%After resource scheduling, the controller decides that: the CPU is already highly utilized in Node~2; the flow comes in (step 1) should traverse the $SDM~1$ data plane instance in Node~1, and data plane of $SDM~2$ and $SDM~3$ in Node~2.
%%
%Correspondingly, it installs rules in Switch 1, steering the flow to Node~1 (step 2).
%%
%Inside $SDM~1$, a process steers the flow through $SDM 1$ data plane (step 3 and 4); the returning flow is further steered to Switch 2 (step 5 and 6); rules are also installed in Switch 2, which steer the flow to Node~2 (step 7).
%%
%In Node~2, the flow traverse $SDM~2$ and $SDM~3$ in sequence (step 8-11); the flow is returned to Switch 2 (step  12) and forward to the rest of the network path (step 13).
%
%\begin{figure}[htbp]
%\centerline{\includegraphics[width=1\linewidth]{figure/chain}}
%\caption{System Diagram} \label{fig:chain}
%\end{figure}

%\presub \subsection{Challenges} \postsub
%%
\noindent\textbf{Challenges:}
%
As mentioned above, there are two challenges for abstraction design: we need to carefully tradeoff between fine and coarse
abstraction granularity, and we need to achieve full programming extensibility.
%
In the following Section~\ref{sec:actions}, we presents the \sys~middlebox data plane abstraction.
%
In Sec~\ref{sec:scheduling},  we solve the service chain scheduling problem.



%%
%\noindent\textbf{Centralization:}







==> chen/related.tex <==
\presec \section{Background and Related Work} \label{sec:related} \postsec
\presub \subsection{Network Function Virtualization} \postsub
%\vspace{0.05in}
%\noindent
%\textbf{Network Function Virtualization:}
%%
Network Function Virtualization wants to address the issues of tight hardware and software coupling and hardware vendor lock-in for middleboxes, by implementing middlebox functions purely in software running on commodity servers~\cite{etsi2012network, etsi2013network}.

However, commodity servers are designed for general computing purposes, not packet processing functions in middleboxes; compared with specialized hardware acceleration, even the best-practise approaches (\eg, based on DPDK and SR-IOV~\cite{inteldata}) still have 10x-50x performance gap~\cite{larkins2015recent}.
%
This is exactly the reason that market has been favoring the closed-but-fast model, which uses proprietary hardware platform with fast packet processing capability, over the open-but-slow model, which uses commodity servers with slow packet processing capability.
%
Even for x86-based data plane, a pure software implementation is not optimal across different hardware configurations:
%
some platforms support high-throughput IO capability (\eg, DPDK~\cite{inteldata}, Netmap~\cite{rizzo2012netmap}), while others do not;
%
some NICs support special computation offload (\eg, TCP checksum offloading, receive side scaling), while others do not;
%
some x86 CPU support special acceleration instructions (\eg, AES instructions~\cite{hoban2010using}), while others do not.

As a result, recent NFV trend calls for an abstraction between the control and data planes~\cite{larkins2015recent}.
%
To be concrete, a normal x86 platform is suitable for general purpose programming, hence it is only effective to serve as the hardware foundation of a light weight NFV data plane.
%
Accelerated platforms (\ie, multi-core CPU, Network Processor, FPGA, GPU or ASIC) are optimized with parallel processing and special network function acceleration, hence should be widely used for high performance data plane processing.
%
\sys~is exactly designed to fill this gap for NFV.
%
%\sys~abstraction significantly simplifies the programming of middlebox functions whereas currently in NFV every middlebox data plane functionality has to be programmed from scratch as NFV does not have such an abstraction layer yet.
\sys~abstraction significantly simplifies the programming of middlebox functions, whereas, currently in NFV every middlebox data plane functionality has to be programmed from scratch as NFV does not have such an abstraction layer yet.

There are some work in NFV focuses on the smooth state transition among commodity servers for middlebox function scale-in and out.
%
These techniques can be used by, and are complementary to, \sys~to support the extensible and manageable data plane.
%
Split/Merge groups middlebox states into \emph{partitioned} and \emph{coherent} and uses an application-level library can help middleboxes manage the state elastically \cite{rajagopalan2013split}.
%
OpenNF uses a combination of events and forwarding updates to address the race condition during the state migration phase \cite{gember2014opennf}.


\presub \subsection{Data Plane Programmability} \postsub
%\vspace{0.05in}
%\noindent
%\textbf{Extensible Router Architecture:}
%
Data plane programmability (both forwarding and function) has gained significant attention.
%
Click is well recognized work along this direction \cite{kohler2000click}.
%
In Click, an \emph{element} is the abstraction of a packet processing operation.
%
Click is not designed for SDN architecture, which has the separation of control/data planes in its core; also, Click is not a platform-independent abstraction.

%
Several systems focus on the data plane throughput of extensible software-based routers.
%
These systems are orthogonal to OpenFunction and they are useful to build OpenFunction boxes.
%
RouteBricks exploits parallelism both across multiple servers and across multiple cores inside each single server ~\cite{dobrescu2009routebricks}.
%
PacketShader exploits the massive parallelism of GPU for batch processing \cite{han2011packetshader}.
%
GASPP focuses on stateful packet processing, and its GPU-accelerated framework can achieve multi-gigabit processing \cite{vasiliadis2014gaspp}.
%
Some systems focus on data plane extensibility of new network forwarding protocols.
%
The main direction is to pair the high-throughput ASIC processing path with a fully programmable co-processer to enhance the programmability.
%
ServerSwitch uses x86 CPU as the co-processor \cite{lu2011serverswitch, lu2012using}.
%
SSDP instead uses an NPU-driven subsystem \cite{narayanan2012macroflows}.
%
SwitchBlade allows rapid prototyping in FPGA \cite{anwer2011switchblade}.


The OpenDataPlane project~\cite{OpenDataPlane} is the most related work.
%
OpenDataPlane is an open-source, cross-platform set of APIs for programming the network processors.
%
Conceptually speaking, \sys~abstraction is higher than OpenDataPlane: similar to P4 in forwarding, \sys~tells the device how to operate, instead of directly manipulating device resources.
%
OpenDataPlane is similar to OpenFlow in forwarding: it needs to deal with threads, cores and memory directly.
%
Even for composing user-defined or not-yet-implemented actions, OpenDataPlane cannot replace the role of our proposed pseudo language: it is dedicated to network processors; while our pseudo language is more general (we demonstrate this later by compiling such a program to a FPGA block).

\presub \subsection{Router Abstraction} \postsub
%\noindent
%\textbf{Router Abstraction:}
%
Some prior work is on designing an abstraction layer to support portability across heterogeneous platforms.
%
Handley \etal built extensible routers on top of commodity platforms in the XORP project \cite{handley2003xorp,handley2005designing}.
%
Their focus is on breaking the complex control plane of routing protocols.
%
XORP significantly differs from OpenFunction.
%
First, XORP is not designed for software-defined networks.
%
Second, the abstraction in XORP focuses on routing whereas the abstraction in OpenFunction focuses middlebox functionalities.
%
Third, in XORP, the extension of the data plane abstraction is still platform-dependent whereas in OpenFunction, the extension of the abstraction is platform-independent by our Ogham language.

%%
Mogul \etal proposed to design an abstraction layer called Orphal to support portability of third-party software among vendor platforms in a position paper \cite{mogul2008api}.
%
Orphal significantly differs from OpenFunction.
%
First, Orphal is not designed for software-defined networks.
%
Second, the abstraction in Orphal is based on router specific hardware resources (such as TCAM and DPI engines) whereas the abstraction in OpenFunction is based on middlebox functionalities.
%
Thus, OpenFunction abstraction supports better hardware heterogeneity than Orphal abstraction because our abstraction is hardware agnostic.
%
Third, similar to XORP, the extension of Orphal abstraction is still platform-dependent whereas in OpenFunction, the extension of the abstraction is platform-independent by our Ogham language.

%%
Song proposed a hardware abstraction called POF, which focuses on protocol-oblivious forwarding  \cite{song2013protocol}.
%
It extends the OpenFlow instructions with protocol-oblivious operations such as \emph{AddField} and \emph{SetFieldFromValue}.
%
Theoretically, a complete set of such low-level primitives can compose any data plane operation; however, using these primitives to construct middlebox functions is extremely difficult because they are too low-level.
%
We have implemented the POF abstraction and used these primitives to implement a NAT, and our experience well confirms the above insight.

%%
Answer \etal discussed the vision of decoupling the processing at the controller and at middleboxes while providing an interface by which they can communicate \cite{anwer2013slick}.
%
This vision is similar to us; however, neither design nor implementation details were given in the two-page position paper \cite{anwer2013slick}.


==> chen/scheduling.tex <==
\presec \section{Service Chain Scheduling} \label{sec:scheduling} \postsec
%
One challenging task for \sys~controllers is to perform service chain scheduling: given a flow and a sequence of SDM functions that the flow needs to pass through, the controller needs to choose a sequence of DP processes of that SDM along the path of the flow so that the flow can go through this sequence of DP processes.
%%
Note that if a specific operation in the program has multiple implementations (\ie, both CPU-based and GPU-based), then the compiled SDM data plane also has multiple implementations.
%
The controller can load any desired implementation according to the resource scheduling and flow requirements.
%
For example, if a middlebox has 3 operations and each operation has 2 implementations; in total there are $2^3=8$ implementations stored for this middlebox.
%
Due to cheap price of hard-drive, we consider this exponential increase in number of implementations a trivial concern.


%
There are some related work in service chain scheduling and enforcement.
%
CoMb exploits consolidation opportunities in NFV deployment to save cost \cite{sekar2012design}.
%
It also provides solutions to resource management, traffic redirection, and coordination among different data plane processing elements.
%
However, it requires that the middlebox processes of the whole service chain pertaining to a given session flow run on the same device.
%
This is not optimal in many \sys~scenarios: image that one hardware platform has special optimization for IPSEC, and another platform has special optimization for cache; force the whole service chain in a single node compromise the NFV benefits of global resource optimization.
%%
Some schemes have been proposed to solve the problem of steering traffic among physical middleboxes to follow the network policy (\ie, service chain).
%
As a pioneer work, the pswitches (\ie, policy-aware switches) scheme adds a new layer-2 for data centers, which can steer the network traffic through unmodified middleboxes \cite{joseph2008policy}.
%
Using SDN, SIMPLE can enforce flow-level policy even if middleboxes modify the packets or change the session level semantics \cite{qazi2013simple}.
%
FlowTag makes a further step by attaching tags to flow packets to enable flow tracking.
%
These existing schemes can be used in \sys~to control the service chain among middlebox platforms \cite{fayazbakhsh2014enforcing}.

%\subsection{Problem Formulation}\label{sec:formu}
%
Table \ref{table:symbols} summarizes the symbols used in this section.
%%
For a given flow, the OpenFunction controller needs the following three types of inputs to perform service chain scheduling.
%
\begin{itemize}
\item \emph{Chaining Requirement:} Each flow has a classification rule that uniquely identifies the flow and estimated bandwidth. For the given flow, we use $SDM_1, SDM_2, \cdots, SDM_K$ to denote the sequence of $K$ SDMs that it needs to traverse. This flow specification is typically specified by network operators.
\item \emph{Implementation Availability:} For each $SDM_k$, let $V_k$ denote the total number of different implementations of $SDM_k$. Each implementation has its specific resource requirement, which is usually multi-dimensional as different actions in an implementation require different resources.
\item \emph{Box Capability:} Let $N$ denote the set of \sys~boxes. Let $\Omega_{n,r}$ denote the capabilities of resource $r$ in each box $n$. Also, the existing utilization of resource $r$ in OpenFunction box $n$ is denoted as $\Gamma_{n,r}$ (in percentage). The OpenFunction controller obtains box capabilities by performing resource monitoring of each OpenFunction box in real time.
\end{itemize}
%
As a practical constraints, all packets in a given flow should traverse the same DP process for a given SDM in the chain.

\begin{table}[htbp]
%\vspace{-0.1in}
\caption{Symbols used in this paper} \label{table:symbols}
\centering
\begin{tabular}{|p{0.8cm}|p{7cm}|}
\hline $k, K$ & SDM k, $1\leq~k\leq~K$. \\
\hline $n, N$ & OpenFunction box n, $1\leq~n\leq~N$. \\
\hline $r, R$ & resource r, $1\leq~r\leq~R$. \\
%\hline $i$ & implementation i. \\
%\hline $f$ & flow f\\
\hline $N_{kl}^f$ & Input binary constant of flow $f$'s service chain to indicate if SDM $l$ is the next SDM of $k$\\
\hline $D_{k,i,r}$ & The amount of resource $r$ is required to support a unit of flow for SDM $k$ with implementation $i$. \\
\hline $\Gamma_{n,r}$ & the existing utilization of resource $r$ in box $n$. \\
\hline $\Omega_{n,r}$ & the capabilities of resource $r$ in box $n$. \\
\hline $A_f$ & The amount of flow $f$\\
\hline $Z_{k,i,n}^{l,j,m,f}$ & Binary variable to indicate if flow $f$ is traversed from the SDM $k$ with implementation $i$ on box $n$ to SDM $l$ with implementation $j$ on box $m$.\\
\hline $X_{k,i,n}$ & The amount of flows traversing node $n$ for SDM $k$ with implementation $i$. \\
\hline
\end{tabular}
\end{table}

\noindent\textbf{ILP Formulation}
The optimization objective in service chain scheduling is load balancing across all resources of all nodes.
%
\begin{equation} \label{equ:obj}
\text{minimize}\ \ \ \ \ \ \ \ \ \ \max \frac{\sum_k \sum_i X_{k,i,n}D_{k,i,r}}{\Omega_{n,r}}+\Gamma_{n,r}
\end{equation}

The main constraint is the flow conservation for each flow crossing the SDMs
\begin{equation} \label{con:flowconservation}
\sum_{l,j,m\geq n}Z_{k,i,n}^{l,j,m,f} - \sum_{l,j,m\leq n}Z_{l,j,m}^{k,i,n,f} = \left\{ \begin{array}{ll}
1 & \textrm{if $k=0,n=0$}\\
-1 & \textrm{if $k=K,n=N$}\\
0 & \textrm{otherwise}
\end{array} \right.
\end{equation}
In addition, a flow may traverse from SDM $k$ to SDM $l$ only if SDM $k$ is followed by SDM $l$ on flow $f$'s service chain,
\begin{equation} \label{con:nextHop}
N_{kl}^f \geq Z_{k,i,n}^{l,j,m,f}
\end{equation}
Based on this flow conservation constraint, the traffic can be calculated by
\begin{equation} \label{con:demandCalcu}
X_{k,i,n}=\sum_{f}\sum_{l,j,m}A_f Z_{l,j,m}^{k,i,n,f}
\end{equation}
To derive an ILP formulation, we can introduce an auxiliary variable $z$ to present the objective function and $z$ should satisfy
\begin{equation} \label{con:auxVariable}
z \geq \frac{\sum_k \sum_i X_{k,i,n}D_{k,i,r}}{\Omega_{n,r}}+\Gamma_{n,r}
\end{equation} \label{equ:finalObj}
and the objective becomes
\begin{equation}
\text{minimize}\ \ \ \ \ \ \ \ \ \  z.
\end{equation}
Therefore, the Integer Linear Programming (ILP) formulation of this problem can be summarized as the resource utilization optimization problem (RUOP).
%minimize \eqref{equ:finalObj}\\
%subject to \eqref{con:flowconservation}, \eqref{con:nextHop}, \eqref{con:demandCalcu}, \eqref{con:auxVariable}
Obviously, the ILP model formulated above is intractable in large size network. 
%
Specifically, due to the large dimension of binary variable $Z_{k,i,n}^{l,j,m,f}$, there will be more than $10^7$ binary variables in the model even if each index has only 10 possible values. 
%
Accordingly, we need to design an efficient heuristic to solve this problem.

%\subsection{Problem Analysis and Algorithm Design}
%\label{subsec:offline}
\noindent\textbf{Offline Algorithm}
We first consider the offline scheduling, where a number of flows are given and can be optimized at one time.
%
Since the most critical element which makes our problem intractable is the large number of binary variables, we consider relaxation and rounding method to solve this problem. 
%
For clear presentation, we call the enforced service chain (\ie, the ordered SDM realized by which box and with which implementation, as the path of this flow. 
%
Following the relaxation and rounding idea, we first relax the binary constraint of the variable $Z_{k,i,n}^{l,j,m,f}$, \ie, treat it as a real variable in the range $[0,1]$, and solve the derived Linear Programming model. 
%
With this solution, each flow may be split among multiple paths which are determined by the value of $Z_{k,i,n}^{l,j,m,f}$. 
%
To get unsplitable path for each flow, a simple method is to directly round each flow to the path which carries the largest fraction of this flow.
%
However, this method cannot obtain a good result especially when there are a lot of boxes and many implementation versions for each SDM. 
%
In this case, each path may carry only a little fraction of the flow; directly rounding each flow to the path carrying maximum fraction of flow may deviate too far away from the ILP optimum. 
%
To solve this problem, we propose a progressive method for the rounding phase to get unsplitable paths.

Respect to progressive rounding, the main idea is to iteratively forbid some links that carrying very little fraction for each flow, till there is only one path for each flow or there is a path carrying most of the fraction of flow. 
%
Based on above discussions, we design Algorithm \ref{alg:offline} to solve the RUOP formualtion.
\begin{algorithm}[t]
\caption{Offline Resource Utilization Optimization}
\label{alg:offline}
\begin{algorithmic}[1]
\REQUIRE Flow volume and service chain requirement, resource requirement for each SDM implementation
\ENSURE The SDM path of each flow
\STATE Formulate RUOP model according to the input
\WHILE {not all $Z_{k,i,n}^{l,j,m,f} = 0 \text{or} 1$}
	\STATE Solve RUOP model
	\STATE Get a forbidden threshold $\epsilon$ \label{lin:threshold}
	\FOR{all $Z_{k,i,n}^{l,j,m,f}$}
		\IF{$Z_{k,i,n}^{l,j,m,f}<\epsilon$}
			\STATE Add one more constraint $Z_{k,i,n}^{l,j,m,f}=0$ into RUOP model
		\ENDIF
	\ENDFOR
\ENDWHILE
\RETURN $\{x_i^k\}$
\end{algorithmic}
\end{algorithm}
In this algorithm, there is one step that has not been discussed.
%
In Line \ref{lin:threshold}, we should find a threshold $\epsilon$ to determine if a $Z_{k,i,n}^{l,j,m,f}$ should be set to 0 for the rounding purpose.
%
This $epsilon$ can be set based on the tradeoff between the algorithm performance and the algorithm running time. With large $epsilon$, more $Z_{k,i,n}^{l,j,m,f}$ will be set to 0 in each loop and hence there are fewer loops will be executed in the algorithm.
%
With smaller $epsilone$, we can do more optimization during the algorithm and hence derive a better solution.
%
On the other hand, we should update the $epsilon$ in each loop since the $Z_{k,i,n}^{l,j,m,f}$ should become larger in each loop as there are fewer paths can be used by the flows with the algorithm execution.
%
Accordingly, without updating the rounding threshold, there will be endless loop in the algorithm.

\noindent\textbf{From Offline to Online}
We can also extend the algorithm to online version of this problem, because in reality
service chain requests may arrive randomly, not all at once.
%
The first scheme is to hold the flows for a while to get a bulk of flows and then trigger the offline algorithm to reserve SDM resources for these flows.
%
If the flow arriving rate is very small, hold flows to wait for the later flows may be a large overhead for the flow arriving earlier.
%
In this case, we can treat each flow as a bulk to trigger Algorithm \ref{alg:offline} to set up SDMs for each single flow. 

==> chen/system.tex <==
\presec \section{Prototype Implementation} \label{sec:system} \postsec
\presub \subsection{Platform} \postsub
%
We build a proof-of-concept system to verify the \sys~abstraction and get an estimation of achievable performance.
%
Existing heterogeneous platforms can serve as the foundation of OpenFunction boxes.
%
Some new platforms are developed specifically for high-throughput software-based middleboxes, such as Intel DPDK \cite{scholz2014look}, Netmap \cite{rizzo2012netmap} and NetSlices \cite{marian2012netslices}.
%
The first two approaches let user space talks to NIC directly, and completely remove the OS stack overhead.
%
NetSlices spatially partitions the hardware resources, and scales linearly with the number of cores.
%
Built on DPDK, NetVM \cite{hwang2014netvm} provides highly efficient inter-VM communication channel for virtualized environments.
%
ClickOS \cite{martins2014clickos} is a Xen-based platform that significantly improves the I/O subsystem; a minimalistic guest VM image is also customized.
%
Also xOMB~\cite{anderson2012xomb} is an open middlebox software architecture.
%
It focus on connection-oriented TCP processing of Internet services.

\noindent\textbf{Data Plane}
%
We develop two kinds of \sys~boxes based on DPDK and Netmap, and one box based on FPGA.
%
Netmap is a tool designed for high speed packet I/O in commodity servers.
%
Implemented as either a modified NIC driver or a kernel module, Netmap also enables high-speed processing in user space.
%
Supported by Intel, Data Plane Development Kit (DPDK) is a combination of data plane libraries and NIC drivers for fast packet processing in user space.
%
Poll mode drivers (PMD) are designed to enable direct packets exchange between a user space process and a NIC.
%
A low overhead \emph{run-to-completion} model is used to achieve fast data plane performance.
%
In our testbed, there are 16 Dell R320 machines, each has a 10G Intel X520-SR1 ethernet NIC and is both DPDK and Netmap enabled.
%
We also develop a prototype box in a FPGA card via Xilinx Vivado High-Level Synthesis tool, which supports C/C++ to describe designs and translates them into hardware description languages (HDL) such as VHDL or Verilog HDL~\cite{meeus2012overview}.
%
The platform is a programmable FPGA card with a Xilinx Kintex 7 chip, two 10 Gbps NIC and four 1 Gbps NIC.

%
For each prototype box, we need to provide three support: \sys~specification, \sys~language and \emph{in-box chain support}.
%
Regards the third requirement, the device needs to support dynamic DP function loading/unloading: consider the scenario initially flow~1 only passes through $SDM~1$ and $SDM~2$, later an operator decides to add an additional action to be performed on that flow and therefore $SDM~3$ is inserted into the service chain.
%
There can be many scenarios for such a need.
%
For example, a company can perform DPI, to block instant message packets (such as gtalk and Skype) only during the office hour.
%
Such temporary insertion/deletion of data plane instances should be seamless as no packet loss is allowed.
%
A simple solution could be to temporarily hold the packets of the flow, construct a new service chain, and switch to the new chain.
%
However, this approach adds significant delay to packets processing during the transition.
%
Instead, we prefer a bufferless solution.
%

\noindent\textbf{Control Plane}
%
OpenFunction controller sends flow steering instructions to the Openflow controller.
%
We use OpenDaylight (ODL) \cite{ortiz2013software} as the OpenFlow controller that manages OpenFlow capable switches and routers.
%%
OpenFunction controller runs as an OpenDaylight application.
%
It uses many base functions provided by ODL to learn about the network and control network elements.

%%
In our testbed, we use OpenvSwitch \cite{ovs} as a switching element to steer traffic.
%
We use a quad core 3.0 GHz 	AMD Phenom(tm) II X4 945 Processor system to host the OpenFunction controller, the OpenFlow controller and all SDM CP processes.

\presub \subsection{Specification Support} \postsub
%
Due to space limitation, we only explain how Netmap-Click and FPGA platforms.
%
DPDK is similar to Netmap-Click.

Netmap tool does not provide enough native packet libraries; therefore, we use Click as the packet processing pipeline and Netmap-enabled \emph{FromDevice/ToDevice} elements for packet processing tasks such as send/recevie.
%
Click has a two-level design: each element class in Click is defined by a pair of .hh/.cc source files; a Click script describes the packet flow graph among different elements.
\begin{algorithm}
\caption{\textbf{Translated Click IPSEC script}}\label{code:clickscript}
in1 :: FromDevice(netmap:eth1, PROMISC true) \;
out2 :: Queue(100) -> ToDevice(netmap:eth2) \;
elementclass ExactMatch Classifier \;
EM::ExactMatch(12/0800,-) \;
\BlankLine
in1->EM->DecapHeader(14)->MyIPsecESPEncap \
->MyAes(1)->IPsecEncap->SetIPChecksum     \
->MarkIPHeader(OFFSET 0)->ChangeSrcIP     \
->ChangeDstIP->EncapHeader->out2 \;
\BlankLine
EM[1]->Discard \;
\end{algorithm}

%
Since the syntax of \sys~specification directly mimics the Click script, this processing is relatively easy.
%
The translated Click script of the IPSEC data plane specification (Algorithm~\ref{code:ipsec}) is shown in Algorithm~\ref{code:clickscript}.
%
One major challenge is the abstract parameters of actions in the specification: we either replace them with real parameters in Click format (\eg, \emph{ExactMatch} in Line 4), or implement them as action attributes, and let the IPSEC CP process sets them in runtime (\eg, \emph{EncapHeader} and \emph{ChangeSrcIP} in Line 5).
%
Another challenge is that we need to add additional \emph{MarkMACHeader} and \emph{MarkIPHeader} elements, after the input device action, for Click specific requirements (Line 5).

In FPGA box, both \sys~specification and pseudo language are translated to the special C/C++ code: the specification is translated to the top level block (composed by a call graph among low level blocks), while each pseudo language based action definition is translated to a low level block.
%
The translation of data plane IPSEC specification (Algorithm~\ref{code:nat}) as shown in Algorithm~\ref{code:fpgatop}, requires
%
(1) defining the inter-link between functional actions (\ie, 5-20); and
%
(2) using direct function calls to represent actions (\eg, Line 21-29).
%
Note that in FPGA platform, we implement all parameters as action attributes, which are controlled by its corresponding CP process.

\begin{algorithm}
\caption{\textbf{Translated Xilinx specification}}\label{code:fpgatop}
void ipsec(stream<axiWord> \&inData, stream<axiWord> \&outData) \{\\
\#pragma HLS dataflow interval=1 \\
\#pragma HLS INTERFACE port=inData axis  \\
\#pragma HLS INTERFACE port=outData axis \\
\BlankLine
	static stream<axiWord> ippacket("ippacket");\\
	static stream<axiWord> decap2espencap("decap2espencap");\\
    static stream<axiWord> espencap2aes("espencap2aes");\\
    static stream<axiWord> aes2ipencap("aes2ipencap");\\
    static stream<axiWord> ipencap2changeSrcIP("ipencap2changeSrcIP");\\
	static stream<axiWord> changeSrcIP2changeDstIP("changeSrcIP2changeDstIP");\\
	static stream<axiWord> changeDstIP2ipchecksum("changeDstIP2ipchecksum");\\
    static stream<axiWord> ipchecksum2macencap("ipchecksum2macencap");\\
\BlankLine
\#pragma HLS STREAM variable=ippacket 		depth=16    \\
\#pragma HLS STREAM variable=decap2espencap 		depth=16  \\
\#pragma HLS STREAM variable=espencap2aes 		depth=16  \\
\#pragma HLS STREAM variable=aes2ipencap 		depth=16  \\
\#pragma HLS STREAM variable=ipencap2changeSrcIP 	depth=16 \\
\#pragma HLS STREAM variable=changeSrcIP2changeDstIP 	depth=16 \\
\#pragma HLS STREAM variable=changeDstIP2ipchecksum depth=16 \\
\#pragma HLS STREAM variable=ipchecksum2macencap depth=16 \\
\BlankLine
	parser(inData, ippacket);\\
	decap(ippacket, decap2espencap);\\
    espencap(decap2espencap, espencap2aes);\\
    aes(espencap2aes,aes2ipencap);\\
    ipencap(aes2ipencap, ipencap2encap);\\
    encap(decap2encap, encap2changeSrcIP);\\
	changeSrcIP(encap2changeSrcIP, changeSrcIP2changeDstIP);\\
    changeDstIP(changeSrcIP2changeDstIP, changeDstIP2ipchecksum);\\
	ipchecksum(changeDstIP2ipchecksum, outData);\\
\}\\
\end{algorithm}

\presub \subsection{Language Support} \postsub
%
In Netmap platform, we translate each action pseudo program to an element class definition in Click.
%
Mostly, the generated codes are in the $simple\_action$ function.
%
Each special line in the pseudo language file is processed.
%
For example, Algorithm~\ref{code:clicksource}~is the translated code of generating a pointer to IP header length field (Algorithm~\ref{alg:SetIPChecksum}~Line 1).
%
Other codes are input from the pseudo program as it is.
%

\begin{algorithm}
\caption{\textbf{Translated Click source}}\label{code:clicksource}
nh\_data = p->network\_header(); \
\BlankLine
unsigned char* pch = NULL \;
pch = nh\_data \;
pch = pch + 0 \;
unsigned char* iphlen = pch \;
\end{algorithm}

%
\sys~language translation in Xilinx FPGA is similar to the operations of that in Netmap-Click.
%
The major difference is that: an additional C++ encapsulation class is required for each action class, to express the state transition semantics in FPGA hardware.
%
Due to space limitation, we omit the details of both FPGA and DPDK platforms in this paper.

\presub \subsection{In-Box Service Chain} \postsub
In this part, we use DPDK to illustrate the provisioning of in-box service chain.
%%
We use process group to realize the service chain and treat each SDM data plane instance as a separate process.
%
As shown in Figure \ref{fig:ioproc}, a single IO process acts as a central process: it sets up all memory structures for use by secondary processes and handles packet reception and transmission.
%
A pair of rings are setup between the IO process and a SDM process for packets exchange.
%
When a new SDM process starts, it discovers both the rings and packet memory locations via DPDK library support.
%
The IO process sends a packet's descriptor through the ring; a SDM data plane processes the packet and returns it via another ring.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tpb]
\centerline{\includegraphics[width=1\linewidth]{figure/ioproc}}
\caption{IO based service chain} \label{fig:ioproc}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
The pair of rings is the key to realize dynamic load/unload.
%
Each packet's metadata carry the service chain information: an array records the indexes of ring pairs it needs to traverse in order, and an index pointer keeps the value of the next pair.
%
Considering the above-mentioned dynamic example, initially only $SDM~1$ and $SDM~2$ are traversed by a flow; later when the new $SDM~3$ data plane process starts, all subsequent packets' metadata change to the new service chain $SDM~1\rightarrow SDM~3\rightarrow SDM~2$; and as a result, packets traverse $SDM~3$ between $SDM~1$ and $SDM~2$.
%
Similarly, to unload a service chain, when $SDM~3$ is removed from the service chain, the metadata of all subsequent packets change to the new service chain $SDM~1\rightarrow SDM~2$ again; the controller waits for a while, before it cleans up the $SDM~3$ process from the system.
%
For performance consideration, we assume all processes of a group is running on a single CPU socket (possibly with multiple cores).
%
Note that multiple process group is supported, if we start different process groups in different sockets.

%
We also support this feature in the FPGA platform.
%
Unlike software, loading/uploading new data plane functions in programmable hardware needs direct support from hardware.
%
Partial Reconfiguration is a feature of modern FPGAs, which allows a subset of the logic fabric of a FPGA to be dynamically reconfigured while the remaining logic continues to
operate \cite{blodget2004partial}.
%
Currently we are still in the process of developing Netmap support of this feature.

\presub \subsection{Developed SDMs} \postsub
%%
We implement NAT and IPSec gateway as two stateless SDMs on all Netmap and FPGA platforms.
%
The NAT middlebox performs simple address translation; the mapping table is stored in its CP process and the mapping item is send to a DP process when the first packeet of a flow comes in.
%
The IPSec gateway uses ESP tunnel model, with AES-EBC encryption.
%
The control plain borrows the code from open-source implementations, and send command to DP processes after security negotiation.

With Netmap, we also implement a simple stateful firewall and a stateful IPS. 
%
The stateful firewall monitors all path-through TCP connections; it removes the allow rules in both directions whenever a RESET flag is detected.
%
The stateful IPS monitors FTP connections: some FTP commands are allowed only after the user authentication; otherwise an alert is raised.

%%
%We use a self-developed TCP packet generator as the sender.
%%
%At receiver, a custom program maintains the throughput stats.


